A Neuro-Symbolic Benchmark Suite for Concept Quality and Reasoning Shortcuts

The advent of powerful neural classifiers has increased interest in problems that require both learning and reasoning. These problems are critical for understanding important properties of models, such as trustworthiness, generalization, interpretability, and compliance to safety and structural constraints. However, recent research observed that tasks requiring both learning and reasoning on background knowledge often suffer from reasoning shortcuts (RSs): predictors can solve the downstream reasoning task without associating the correct concepts to the high-dimensional data. To address this issue, we introduce rsbench, a comprehensive benchmark suite designed to systematically evaluate the impact of RSs on models by providing easy access to highly customizable tasks affected by RSs. Furthermore, rsbench implements common metrics for evaluating concept quality and introduces novel formal verification procedures for assessing the presence of RSs in learning tasks. Using rsbench, we highlight that obtaining high quality concepts in both purely neural and neuro-symbolic models is a far-from-solved problem. rsbench is available at: https://unitn-sml.github.io/rsbench.

==> figures/generative-process.tex <==
\begin{tikzpicture}[
            scale=1,
            transform shape,
            node distance=.25cm and .75cm,
            minimum width={width("G")+15pt},
            minimum height={width("G")+15pt},
            mynode/.style={draw,ellipse,align=center}
            ]

            \node[mynode, ] (G) {$\vG$};
            \node[mynode, fill=black!13!white, below left=of G] (X) {$\vX$};
            \node[mynode, below right=of G, fill=black!13!white] (Y) {$\vY$};
            \node[mynode, below right=of X, blue, dashed] (C) {$\vC$};
                
            % \path
            %     (G) edge[-latex] (X)
            %     (G) edge[-latex] (Y)
            %     (Y) edge[-latex] (C);
            
            \draw [->] (G) -- (Y);
            \draw [->] (G) -- (X);
            \draw [->, blue] (X) -- (Y);
            % \draw [->, bend angle=45, bend left, dashed, red] (Y) to node[below, pos=.75] {\textcolor{red}{$f$}} (G);
            % \draw [->] (G) to node[above, pos=.5] {\textcolor{red}{$\beta_\BK$}} (X);
            \draw [->, blue, dashed] (C) to (Y);
            \draw [->, blue, dashed] (X) to (C);
            % \draw [->, bend angle=60, bend left, dashed, magenta] (G) to (C); %to node[above, pos=.9] {{$\alpha$}} (C);
        \end{tikzpicture}

==> tables/boia.tex <==
\scalebox{.9}{
\begin{tabular}{lcccccccccc}
    \toprule
        & \textsc{$\mYAcc$}
        & \textsc{$\mFY$}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
        & \textsc{$\FCollapse$}
        & \textsc{$\SCollapse$}
        & \textsc{$\LCollapse$}
        & \textsc{$\RCollapse$}
    \\
    \midrule
    \DPL & $0.74 \pm 0.02$ & $0.69 \pm 0.03$ & $0.65 \pm 0.01$ & $0.44 \pm 0.01$ & $0.88 \pm 0.01$ & $0.52 \pm 0.01$ & $0.67 \pm 0.01$ & $0.71 \pm 0.09$ & $0.68 \pm 0.07$ & $0.30 \pm 0.02$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.72 \pm 0.05$ & $0.68 \pm 0.05$ & $0.78 \pm 0.01$ & $0.54 \pm 0.01$ & $0.95 \pm 0.02$ & $0.66 \pm 0.06$ & $0.67 \pm 0.01$ & $0.78 \pm 0.01$ & $0.56 \pm 0.11$ & $0.68 \pm 0.04$
    \\
    \SymCBM & $0.68 \pm 0.02$ & $0.63 \pm 0.02$ & $0.68 \pm 0.01$ & $0.53 \pm 0.02$ & $0.41 \pm 0.02$ & $0.25 \pm 0.01$ & $0.00 \pm 0.01$ & $0.58 \pm 0.07$ & $0.15 \pm 0.05$ & $0.15 \pm 0.05$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.69 \pm 0.01$ & $0.64 \pm 0.01$ & $0.46 \pm 0.07$ & $0.37 \pm 0.04$ & $0.22 \pm 0.05$ & $0.43 \pm 0.04$ & $0.30 \pm 0.11$ & $0.29 \pm 0.11$ & $0.13 \pm 0.05$ & $0.28 \pm 0.12$
    \\
    \SymCLIP & $0.84 \pm 0.05$ & $0.77 \pm 0.06$ & $0.44 \pm 0.06$ & $0.37 \pm 0.04$ & $0.89 \pm 0.03$ & $0.57 \pm 0.05$ & $0.52 \pm 0.24$ & $0.62 \pm 0.10$ & $0.57 \pm 0.03$ & $0.83 \pm 0.09$
    \\
    \bottomrule
\end{tabular}
}

==> tables/kand.tex <==
%\scalebox{.9}{
% \begin{tabular}{lcccccc}
%     \toprule
%         & \textsc{$\YAcc$}
%         & \textsc{$\FY$}
%         & \textsc{$\CAcc$}
%         & \textsc{$\FC$}
%         & \textsc{$\Collapse$}
%         & \textsc{$\HCollapse$}
%     \\
%     \midrule
%     \DPL & $0.87 \pm 0.16$ & $0.87 \pm 0.16$ & $0.29 \pm 0.09$ & $0.26 \pm 0.10$ & $0.71 \pm 0.05$ & $0.58 \pm 0.10$
%     \\
%     \rowcolor[HTML]{EFEFEF}
%     \LTN & $0.66 \pm 0.09$ &  $0.64 \pm 0.10$ & $0.34 \pm 0.04$ & $0.34 \pm 0.04$ & $0.00 \pm 0.01$ & $0.20 \pm 0.17$
%     \\
%     \NN & $0.72 \pm 0.08$ & $0.72 \pm 0.08$ & $-$ & $-$ & $-$ & $-$
%     \\
%     \rowcolor[HTML]{EFEFEF}
%     \CBM & $0.52 \pm 0.01$ & $0.52 \pm 0.01^\dagger$ & $0.98 \pm 0.07^\dagger$ & $0.98 \pm 0.8^\dagger$ & $0.01 \pm 0.01^\dagger$ & $0.01 \pm 0.01\dagger$
%     \\
%     \CLIP  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$
%     \\
%     \bottomrule
% \end{tabular}

\begin{tabular}{lcccccc}
    \toprule
        & \textsc{$\YAcc$}
        & \textsc{$\FY$}
        & \textsc{$\CAcc$}
        & \textsc{$\FC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \DPL & $0.87 \pm 0.15$ & $0.87 \pm 0.15$ & $0.28 \pm 0.09$ & $0.25 \pm 0.09$ & $0.69 \pm 0.04$ & $0.54 \pm 0.08$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.78 \pm 0.09$ & $0.77 \pm 0.09$ & $0.35 \pm 0.04$ & $0.35 \pm 0.04$ & $0.00 \pm 0.01$ & $0.14 \pm 0.16$
    \\
    \SymCBM & $0.50 \pm 0.01$ & $0.36 \pm 0.04$ & $0.59 \pm 0.01$ & $0.59 \pm 0.01$ & $0.00 \pm 0.01$ & $0.01 \pm 0.01$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.72 \pm 0.08$ & $0.72 \pm 0.08$ & $0.33 \pm 0.01$ & $0.17 \pm 0.01$ & $0.89 \pm 0.01$ & $0.99 \pm 0.01$
    \\
    \SymCLIP & $0.99 \pm 0.01$ & $0.99 \pm 0.01$ & $0.34 \pm 0.01$ & $0.32 \pm 0.01$ & $0.00 \pm 0.01$ & $0.08 \pm 0.03$
    \\
    \bottomrule
\end{tabular}
%}

% OLD PERFORMANCES KAND: full sup
% $0.51 \pm 0.01$ & $0.51 \pm 0.01$ & $0.99 \pm 0.01^\dagger$ & $0.99 \pm 0.01^\dagger$ & $0.00 \pm 0.01^\dagger$ & $0.01 \pm 0.01^\dagger$

% Performances with partial supervision (square, red and circle)
%Concept Accuracy (In): $0.59 \pm 0.00$
%Label Accuracy (In): $0.50 \pm 0.00$
%Concept F1 Macro (In): $0.59 \pm 0.00$
%Concept F1 Micro (In): $0.59 \pm 0.00$
%Concept F1 Weighted (In): $0.59 \pm 0.00$
%Label F1 Macro (In): $0.36 \pm 0.04$
%Label F1 Micro (In): $0.50 \pm 0.00$
%Label F1 Weighted (In): $0.36 \pm 0.04$
%Collapse (In): $0.00 \pm 0.00$
%Collapse Hard (In): $0.01 \pm 0.00$
%Avg Nll (In): $0.70 \pm 0.00$
%Collapse Shapes (In): $0.00 \pm 0.00$
%Collapse Hard Shapes (In): $0.01 \pm 0.00$
%Collapse Color (In): $0.00 \pm 0.00$
%Collapse Hard Color (In): $0.00 \pm 0.00$
%Mean Collapse (In): $0.00 \pm 0.00$

==> tables/miniboia-ood-ambulance.tex <==
\scalebox{.9}{
\begin{tabular}{lcccccccccc}
    \toprule
        & \textsc{$\mYAcc$}
        & \textsc{$\mFY$}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
        & \textsc{$\FCollapse$}
        & \textsc{$\SCollapse$}
        & \textsc{$\LCollapse$}
        & \textsc{$\RCollapse$}
    \\
    \midrule
    \DPL & $0.70 \pm 0.07$ & $0.62 \pm 0.09$ & $0.61 \pm 0.02$ & $0.54 \pm 0.02$ & $0.37 \pm 0.06$ & $0.35 \pm 0.04$ & $0.77 \pm 0.05$ & $0.00 \pm 0.01$ & $0.55 \pm 0.14$ & $0.62 \pm 0.13$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.74 \pm 0.07$ & $0.72 \pm 0.06$ & $0.68 \pm 0.02$ & $0.51 \pm 0.02$ & $0.32 \pm 0.04$ & $0.33 \pm 0.04$ & $0.60 \pm 0.01$ & $0.00 \pm 0.01$ & $0.56 \pm 0.06$ & $0.62 \pm 0.06$
    \\
    \SymCBM & $0.46 \pm 0.05$ & $0.45 \pm 0.05$ & $0.76 \pm 0.03$ & $0.61 \pm 0.04$ & $0.32 \pm 0.05$ & $0.55 \pm 0.04$ & $0.26 \pm 0.18$ & $0.00 \pm 0.01$ & $0.40 \pm 0.06$ & $0.37 \pm 0.08$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.56 \pm 0.21$ & $0.47 \pm 0.19$ & $0.50 \pm 0.04$ & $0.45 \pm 0.04$ & $0.24 \pm 0.36$ & $0.29 \pm 0.36$ & $0.15 \pm 0.30$ & $0.11 \pm 0.20$ & $0.27 \pm 0.33$ & $0.29 \pm 0.32$
    \\
    \SymCLIP & $0.82 \pm 0.05$ & $0.81 \pm 0.06$ & $0.53 \pm 0.03$ & $0.49 \pm 0.03$ & $0.05 \pm 0.01$ & $0.09 \pm 0.03$ & $0.00 \pm 0.01$ & $0.01 \pm 0.01$ & $0.13 \pm 0.04$ & $0.12 \pm 0.06$
    \\
    \bottomrule
\end{tabular}
}

==> tables/miniboia-ood-only-imgs.tex <==
\scalebox{.9}{
\begin{tabular}{lcccccccccc}
    \toprule
        & \textsc{$\mYAcc$}
        & \textsc{$\mFY$}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
        & \textsc{$\FCollapse$}
        & \textsc{$\SCollapse$}
        & \textsc{$\LCollapse$}
        & \textsc{$\RCollapse$}
    \\
    \midrule
    \DPL & $0.66 \pm 0.08$ & $0.64 \pm 0.08$ & $0.60 \pm 0.02$ & $0.53 \pm 0.02$ & $0.37 \pm 0.06$ & $0.34 \pm 0.04$ & $0.77 \pm 0.05$ & $0.00 \pm 0.01$ & $0.55 \pm 0.13$ & $0.62 \pm 0.13$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.69 \pm 0.06$ & $0.66 \pm 0.06$ & $0.67 \pm 0.01$ & $0.50 \pm 0.02$ & $0.32 \pm 0.04$ & $0.33 \pm 0.04$ & $0.60 \pm 0.00$ & $0.00 \pm 0.01$ &  $0.55 \pm 0.05$ & $0.61 \pm 0.07$
    \\
    \SymCBM & $0.56 \pm 0.04$ & $0.56 \pm 0.04$ & $0.75 \pm 0.03$ & $0.58 \pm 0.05$ & $0.31 \pm 0.06$ & $0.55 \pm 0.04$ & $0.23 \pm 0.20$ & $0.00 \pm 0.01$ & $0.40 \pm 0.07$ & $0.38 \pm 0.10$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.52 \pm 0.19$ & $0.42 \pm 0.17$ & $0.47 \pm 0.02$ & $0.41 \pm 0.01$ & $0.24 \pm 0.36$ & $0.29 \pm 0.36$ & $0.18 \pm 0.31$ & $0.11 \pm 0.20$ & $0.27 \pm 0.33$ & $0.26 \pm 0.33$
    \\
    \SymCLIP & $0.95 \pm 0.02$ & $0.95 \pm 0.02$ & $0.50 \pm 0.03$ & $0.46 \pm 0.02$ & $0.04 \pm 0.01$ & $0.07 \pm 0.02$ & $0.00 \pm 0.01$ & $0.01 \pm 0.01$ & $0.08 \pm 0.03$ & $0.13 \pm 0.06$
    \\
    \bottomrule
\end{tabular}
}

==> tables/miniboia.tex <==
\scalebox{.9}{
\begin{tabular}{lcccccccccc}
    \toprule
        & \textsc{$\mYAcc$}
        & \textsc{$\mFY$}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
        & \textsc{$\FCollapse$}
        & \textsc{$\SCollapse$}
        & \textsc{$\LCollapse$}
        & \textsc{$\RCollapse$}
    \\
    \midrule
    \DPL & $0.81 \pm 0.01$ & $0.80 \pm 0.01$ & $0.57 \pm 0.04$ & $0.49 \pm 0.03$ & $0.86 \pm 0.04$ & $0.55 \pm 0.03$ & $0.84 \pm 0.06$ & $0.78 \pm 0.08$ & $0.72 \pm 0.11$ & $0.79 \pm 0.08$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.85 \pm 0.03$ & $0.82 \pm 0.04$ & $0.64 \pm 0.03$ & $0.46 \pm 0.04$ & $0.81 \pm 0.02$ & $0.46 \pm 0.02$ & $0.75 \pm 0.01$ & $0.91 \pm 0.01$ & $0.75 \pm 0.04$ & $0.77 \pm 0.04$
    \\
    \SymCBM & $0.64 \pm 0.11$ & $0.60 \pm 0.12$ & $0.70 \pm 0.03$ & $0.61 \pm 0.04$ & $0.68 \pm 0.06$ & $0.44 \pm 0.03$ & $0.20 \pm 0.22$ & $0.52 \pm 0.11$ & $0.52 \pm 0.06$ & $0.49 \pm 0.14$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.93 \pm 0.17$ & $0.93 \pm 0.18$ & $0.49 \pm 0.02$ & $0.44 \pm 0.02$ & $0.43 \pm 0.28$ & $0.31 \pm 0.34$ & $0.18 \pm 0.35$ & $0.23 \pm 0.37$ & $0.36 \pm 0.31$ & $0.29 \pm 0.34$
    \\
    \SymCLIP & $0.92 \pm 0.07$ & $0.90 \pm 0.09$ & $0.47 \pm 0.03$ & $0.43 \pm 0.04$ & $0.23 \pm 0.02$ & $0.09 \pm 0.01$ & $0.00 \pm 0.01$ & $0.18 \pm 0.07$ & $0.12 \pm 0.08$ & $0.26 \pm 0.05$ \\
    \bottomrule
\end{tabular}
}

% OLD RESULTS, full supervision
% $0.82 \pm 0.08$ & $0.81 \pm 0.09$ & $0.85 \pm 0.01$ & $0.78 \pm 0.02$ & $0.41 \pm 0.04$ & $0.20 \pm 0.02$ & $0.00 \pm 0.01$ & $0.45 \pm 0.08$ & $0.41 \pm 0.13$ & $0.30 \pm 0.10$

% new results, sup only on certain objects
% Concept Accuracy (In): $0.70 \pm 0.03$
% Concept Accuracy (OOD): $0.75 \pm 0.03$
% Label Accuracy (In): $0.64 \pm 0.11$
% Label Accuracy (OOD): $0.56 \pm 0.04$
%Concept F1 Macro (In): $0.61 \pm 0.04$
%Concept F1 Macro (OOD): $0.58 \pm 0.05$
%Concept F1 Micro (In): $0.70 \pm 0.03$
%Concept F1 Micro (OOD): $0.75 \pm 0.03$
%Concept F1 Weighted (In): $0.70 \pm 0.03$
%Concept F1 Weighted (OOD): $0.72 \pm 0.03$
%Label F1 Macro (In): $0.60 \pm 0.12$
%Label F1 Macro (OOD): $0.56 \pm 0.04$
%Label F1 Micro (In): $0.64 \pm 0.11$
%Label F1 Micro (OOD): $0.56 \pm 0.04$
%Label F1 Weighted (In): $0.63 \pm 0.11$
%Label F1 Weighted (OOD): $0.57 \pm 0.04$
%Collapse (In): $0.68 \pm 0.06$
%Collapse (OOD): $0.31 \pm 0.06$
%Collapse Hard (In): $0.44 \pm 0.03$
%Collapse Hard (OOD): $0.55 \pm 0.04$
%Collapse Forward (In): $0.20 \pm 0.22$
%Collapse Forward (OOD): $0.23 \pm 0.20$
%Collapse Stop (In): $0.52 \pm 0.11$
%Collapse Stop (OOD): $0.00 \pm 0.00$
%Collapse Left (In): $0.52 \pm 0.06$
%Collapse Left (OOD): $0.40 \pm 0.07$
%Collapse Right (In): $0.49 \pm 0.14$
%Collapse Right (OOD): $0.38 \pm 0.10$
%Collapse Hard Forward (In): $0.31 \pm 0.13$
%Collapse Hard Forward (OOD): $0.52 \pm 0.08$
%Collapse Hard Stop (In): $0.63 \pm 0.05$
%Collapse Hard Stop (OOD): $0.84 \pm 0.04$
%Collapse Hard Left (In): $0.42 \pm 0.04$
%Collapse Hard Left (OOD): $0.59 \pm 0.05$
%Collapse Hard Right (In): $0.40 \pm 0.04$
%Collapse Hard Right (OOD): $0.55 \pm 0.05$


==> tables/mnist-ood.tex <==
%\scalebox{.9}{
\begin{tabular}{lcccccc}
    \toprule
        & \textsc{$\YAcc (\uparrow)$}
        & \textsc{$\FY (\uparrow)$}
        & \textsc{$\CAcc (\uparrow)$}
        & \textsc{$\FC (\uparrow)$}
        & \textsc{$\Collapse (\downarrow)$}
        & \textsc{$\HCollapse (\downarrow)$}
    \\
    \midrule
    \DPL & $0.07 \pm 0.04$ & $0.04 \pm 0.04$ & $0.09 \pm 0.14$ & $0.05 \pm 0.08$ & $0.56 \pm 0.05$ & $0.47 \pm 0.08$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.11 \pm 0.13$ & $0.03 \pm 0.03$ & $0.11 \pm 0.13$ & $0.06 \pm 0.07$ & $0.70 \pm 0.01$ & $0.56 \pm 0.03$
    \\
    \SymCBM & $0.01 \pm 0.01$ & $0.00 \pm 0.01$ & $0.50 \pm 0.06$ & $0.43 \pm 0.07$ & $0.08 \pm 0.10$ & $0.15 \pm 0.05$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.02 \pm 0.03$ & $0.00 \pm 0.01$ &  $-$ & $-$ & $-$ & $-$
    \\
    \SymCLIP & $0.00 \pm 0.01$ & $0.00 \pm 0.01$ & $0.12 \pm 0.03$ & $0.06 \pm 0.02$ & $0.46 \pm 0.20$ & $0.42 \pm 0.17$
    \\
    \bottomrule
\end{tabular}
%}

==> tables/mnistshort.tex <==
%\scalebox{.9}{
%\begin{tabular}{lcccccc}
%    \toprule
%        & \textsc{$\YAcc (\uparrow)$}
%        & \textsc{$\FY (\uparrow)$}
%        & \textsc{$\CAcc (\uparrow)$}
%        & \textsc{$\FC (\uparrow)$}
%        & \textsc{$\Collapse (\downarrow)$}
%        & \textsc{$\HCollapse (\downarrow)$}
%    \\
%    \midrule
%    \DPL & $0.97 \pm 0.04$ & $0.62 \pm 0.19$ & $0.06 \pm 0.12$ & $0.04 \pm 0.07$ & $0.48 \pm 0.07$ & $0.52 \pm 0.06$
%    \\
%    \rowcolor[HTML]{EFEFEF}
%    \LTN & $0.80 \pm 0.12$ & $0.43 \pm 0.10$ & $0.06 \pm 0.09$ & $0.03 \pm 0.04$ & $0.70 \pm 0.01$ & $0.60 \pm 0.03$
%    \\
%    \NN & $0.67 \pm 0.30$ & $0.58 \pm 0.37$ & $0.11 \pm 0.02$ & $0.07 \pm 0.03$ & $0.29 \pm 0.34$ & $0.41 \pm 0.26$
%    \\
%    \rowcolor[HTML]{EFEFEF}
%    \CBM & $0.92 \pm 0.13$ & $0.90 \pm 0.18$ & $0.51 \pm 0.07$ & $0.43 \pm 0.08$ & $0.04 \pm 0.05$ & $0.16 \pm 0.02$
%    \\
%    \CLIP  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$
%    \\
%    \bottomrule
%\end{tabular}

\begin{tabular}{lcccccc}
    \toprule
        & \textsc{$\YAcc (\uparrow)$}
        & \textsc{$\FY (\uparrow)$}
        & \textsc{$\CAcc (\uparrow)$}
        & \textsc{$\FC (\uparrow)$}
        & \textsc{$\Collapse (\downarrow)$}
        & \textsc{$\HCollapse (\downarrow)$}
    \\
    \midrule
    \DPL & $0.95 \pm 0.04$ & $0.94 \pm 0.04$ & $0.09 \pm 0.14$ & $0.06 \pm 0.08$ & $0.61 \pm 0.08$ & $0.51 \pm 0.07$
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.89 \pm 0.12$ & $0.66 \pm 0.10$ & $0.10 \pm 0.12$ & $0.05 \pm 0.06$ & $0.70 \pm 0.01$ & $0.58 \pm 0.05$
    \\
    \SymCBM & $0.90 \pm 0.09$ & $0.89 \pm 0.13$ & $0.52 \pm 0.05$ & $0.44 \pm 0.07$ & $0.09 \pm 0.09$ & $0.19 \pm 0.05$
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.67 \pm 0.31$ & $0.57 \pm 0.38$ & $0.11 \pm 0.02$ & $0.07 \pm 0.03$ & $0.29 \pm 0.34$ & $0.41 \pm 0.26$
    \\
    \SymCLIP & $0.66 \pm 0.05$ & $0.62 \pm 0.14$ & $0.08 \pm 0.02$ & $0.04 \pm 0.01$ & $0.48 \pm 0.17$ & $0.46 \pm 0.13$
    \\
    \bottomrule
\end{tabular}
%}

==> tables/short-boia.tex <==
\scalebox{1}{
\begin{tabular}{lccc}
    \toprule
        & \textsc{$\mFY$}
        & \textsc{$\mFC$}
        & m-\textsc{$\Collapse$}
    \\
    \midrule
    \DPL & $0.69 \pm 0.03$ & $0.44 \pm 0.01$ & $0.88 \pm 0.01$ 
    \\
    \rowcolor[HTML]{EFEFEF}
    \LTN & $0.68 \pm 0.05$ & $0.54 \pm 0.01$ & $0.95 \pm 0.02$ 
    \\
    \SymCBM & $0.69 \pm 0.06$ & $0.69 \pm 0.03$ & $0.43 \pm 0.09$ 
    \\
    \rowcolor[HTML]{EFEFEF}
    \SymNN & $0.64 \pm 0.01$ & $0.37 \pm 0.04$ & $0.22 \pm 0.05$ 
    \\
    \SymCLIP & $0.77 \pm 0.06$ & $0.37 \pm 0.04$ & $0.89 \pm 0.03$ 
    \\
    \bottomrule
\end{tabular}
}

==> tables/tcav/nn/boia.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$fc_1$} & $1$ & $0.44 \pm 0.04$ & $0.36 \pm 0.03$ & $0.08 \pm 0.05$ & $0.23 \pm 0.13$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc_2$} & $2$ & $0.50 \pm 0.04$ & $0.39 \pm 0.03$ & $0.15 \pm 0.01$ & $0.35 \pm 0.03$ \\
    \textsc{$fc_3$} & $3$ & $0.48 \pm 0.05$ & $0.38 \pm 0.03$ & $0.18 \pm 0.03$ & $0.37 \pm 0.02$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc_4$} & $4$ & $0.46 \pm 0.07$ & $0.37 \pm 0.04$ & $0.22 \pm 0.05$ &  $0.43 \pm 0.04$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/clipboia.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$fc_1$} & $1$ & $0.50 \pm 0.02$ & $0.41 \pm 0.02$ & $0.22 \pm 0.05$ & $0.10 \pm 0.04$  \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc_2$} & $2$ & $0.55 \pm 0.04$ & $0.44 \pm 0.05$ & $0.43 \pm 0.12$ & $0.25 \pm 0.07$\\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/clipkand.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\CAcc$}
        & \textsc{$\FC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$fc1$} & $1$ & $0.33 \pm 0.01$ & $0.32 \pm 0.01$ & $0.00 \pm 0.01$ & $0.06 \pm 0.03$\\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc2$} & $2$ & $0.34 \pm 0.01$ & $0.32 \pm 0.01$ & $0.00 \pm 0.01$ & $0.10 \pm 0.08$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/clipminiboia.tex <==
\SB{Work in progress...}

==> tables/tcav/nn/clipmnist.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\CAcc$}
        & \textsc{$\FC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$fc1$} & $1$ & $0.11 \pm 0.03$ & $0.07 \pm 0.03$ & $0.52 \pm 0.17$ & $0.47 \pm 0.09$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc2$} & $2$ & $0.09 \pm 0.03$ & $0.05 \pm 0.02$ & $0.54 \pm 0.15$ & $0.45 \pm 0.11$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/kand.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\CAcc$}
        & \textsc{$\FC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$conv1$} & $1$ & $0.35 \pm 0.01$ & $0.34 \pm 0.01$ & $0.00 \pm 0.01$ & $0.02 \pm 0.01$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv2$} & $2$ & $0.35 \pm 0.01$ & $0.34 \pm 0.01$ & $0.00 \pm 0.01$ & $0.02 \pm 0.01$ \\
    \textsc{$conv3$} & $3$ & $0.34 \pm 0.01$ & $0.34 \pm 0.01$ & $0.00 \pm 0.01$ & $0.02 \pm 0.01$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv4$} & $4$ & $0.35 \pm 0.01$ & $0.34 \pm 0.01$ & $0.00 \pm 0.01$ & $0.03 \pm 0.01$ \\
    \textsc{$conv5$} & $5$ & $0.35 \pm 0.01$ & $0.34 \pm 0.01$ & $0.00 \pm 0.01$ & $0.05 \pm 0.02$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc1$} & $6$ & $0.33 \pm 0.01$ & $0.32 \pm 0.01$ & $0.00 \pm 0.01$ & $0.06 \pm 0.03$ \\
    \textsc{$fc2$} & $7$ & $0.33 \pm 0.01$ & $0.31 \pm 0.01$ & $0.00 \pm 0.01$ & $0.12 \pm 0.05$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/miniboia.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$conv1$} & $1$ & $0.48 \pm 0.02$ & $0.44 \pm 0.01$ & $0.19 \pm 0.05$ & $0.07 \pm 0.06$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv2$} & $2$ & $0.49 \pm 0.02$ & $0.45 \pm 0.02$ & $0.20 \pm 0.06$ & $0.08 \pm 0.06$ \\
    \textsc{$conv3$} & $3$ & $0.49 \pm 0.03$ & $0.45 \pm 0.03$ & $0.21 \pm 0.09$ & $0.09 \pm 0.08$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv4$} & $4$ & $0.48 \pm 0.02$ & $0.44 \pm 0.01$ & $0.23 \pm 0.15$ & $0.10 \pm 0.11$ \\
    \textsc{$conv5$} & $5$ & $0.48 \pm 0.02$ & $0.44 \pm 0.02$ & $0.30 \pm 0.26$ & $0.16 \pm 0.23$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv6$} & $6$ & $0.46 \pm 0.02$ & $0.43 \pm 0.02$ & $0.34 \pm 0.33$ & $0.25 \pm 0.38$ \\
    \textsc{$fc1$} & $7$ & $0.50 \pm 0.02$ & $0.45 \pm 0.03$ & $0.38 \pm 0.31$ & $0.28 \pm 0.36$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc2$} & $8$ & $0.49 \pm 0.02$ & $0.44 \pm 0.02$ & $0.43 \pm 0.28$ & $0.31 \pm 0.34$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/miniboia_synth.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\mCAcc$}
        & \textsc{$\mFC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$conv1$} & $1$ & $0.47 \pm 0.02$ & $0.43 \pm 0.02$ & $0.18 \pm 0.03$ & $0.05 \pm 0.03$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv2$} & $2$ & $0.48 \pm 0.02$ & $0.44 \pm 0.02$ & $0.18 \pm 0.03$ & $0.06 \pm 0.03$ \\
    \textsc{$conv3$} & $3$ & $0.49 \pm 0.01$ & $0.45 \pm 0.01$ & $0.23 \pm 0.12$ & $0.09 \pm 0.09$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv4$} & $4$ & $0.48 \pm 0.03$ & $0.44 \pm 0.03$ & $0.23 \pm 0.14$ & $0.13 \pm 0.16$ \\
    \textsc{$conv5$} & $5$ & $0.48 \pm 0.02$ & $0.44 \pm 0.02$ & $0.29 \pm 0.25$ & $0.14 \pm 0.19$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv6$} & $6$ & $0.48 \pm 0.04$ & $0.45 \pm 0.04$ & $0.34 \pm 0.32$ & $0.18 \pm 0.23$ \\
    \textsc{$fc1$} & $7$ & $0.51 \pm 0.03$ & $0.45 \pm 0.03$ & $0.38 \pm 0.31$ & $0.28 \pm 0.36$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc2$} & $8$ & $0.74 \pm 0.01$ & $0.42 \pm 0.01$ & $0.99 \pm 0.01$ & $0.99 \pm 0.01$ \\
    \bottomrule
\end{tabular}
%}

==> tables/tcav/nn/mnistshort.tex <==
%\scalebox{.9}{
\begin{tabular}{lccccc}
    \toprule
        & \textsc{Layer Num}
        & \textsc{$\CAcc$}
        & \textsc{$\FC$}
        & \textsc{$\Collapse$}
        & \textsc{$\HCollapse$}
    \\
    \midrule
    \textsc{$conv_1$} & $1$ & $0.11 \pm 0.03$ & $0.10 \pm 0.03$ & $0.00 \pm 0.00$ & $0.08 \pm 0.05$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$conv_2$} & $2$ & $0.12 \pm 0.03$ & $0.10 \pm 0.04$ & $0.01 \pm 0.02$ & $0.15 \pm 0.04$ \\
    \textsc{$fc_1$} & $3$ & $0.12 \pm 0.04$ & $0.09 \pm 0.05$ & $0.24 \pm 0.30$ & $0.34 \pm 0.26$ \\
    \rowcolor[HTML]{EFEFEF}
    \textsc{$fc_2$} & $4$ & $0.11 \pm 0.02$ & $0.07 \pm 0.03$ & $0.29 \pm 0.34$ &  $0.41 \pm 0.26$ \\
    \bottomrule
\end{tabular}
%}
